Energy-Latency Attacks via Sponge Poisoning

Sponge examples are test-time inputs optimized to increase energy consumption and prediction latency of deep networks deployed on hardware accelerators. By increasing the fraction of neurons activated during classification, these attacks reduce sparsity in network activation patterns, worsening the performance of hardware accelerators. In this work, we present a novel training-time attack, named sponge poisoning, which aims to worsen energy consumption and prediction latency of neural networks on any test input without affecting classification accuracy. To stage this attack, we assume that the attacker can control only a few model updates during training -- a likely scenario, e.g., when model training is outsourced to an untrusted third party or distributed via federated learning. Our extensive experiments on image classification tasks show that sponge poisoning is effective, and that fine-tuning poisoned models to repair them poses prohibitive costs for most users, highlighting that tackling sponge poisoning remains an open issue.

==> commands.tex <==
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{hyperref}

\usepackage{tikz}
\usepackage{comment}
\usepackage{amsmath,amssymb} % define this before the line numbering.
\usepackage{color}
\usepackage{wrapfig}

\newcommand\set[1]{\mathcal{#1}}
\newcommand*\rotvertical{\rotatebox{90}}

\newcommand{\myparagraph}[1]{\noindent \textbf{#1}}
\newcommand{\textitparagraph}[1]{\noindent \paragraph{#1}}

\newcommand{\mycomment}[1]{\textcolor{red}{#1}}

\newcommand{\vct}[1]{\boldsymbol{\ensuremath{#1}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\bigo}{\mathcal{O}}
\usepackage{xcolor}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}

\newcommand{\expnumber}[2]{\ensuremath{{#1}\mathrm{e}{#2}}}
\newcommand{\nexp}[1]{\ensuremath{1\mathrm{e}{-#1}}}

\usepackage{array}

\newcolumntype{?}{!{\vrule width 1pt}}

%%% Coloring the comment as blue
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}

